Measurement of $\phi$ meson production in p+p interactions at 40, 80 and 158 GeV/c with the NA61/SHINE spectrometer at the CERN SPS

Results on $\phi$ meson production in inelastic p+p collisions at CERN SPS energies are presented. They are derived from data collected by the NA61/SHINE fixed target experiment, by means of invariant mass spectra fits in the $\phi \to K^+K^-$ decay channel. They include the first ever measured double differential spectra of $\phi$ mesons as a function of rapidity $y$ and transverse momentum $p_T$ for proton beam momenta of 80 GeV/c and 158 GeV/c, as well as single differential spectra of $y$ or $p_T$ for beam momentum of 40 GeV/c. The corresponding total $\phi$ yields per inelastic p+p event are obtained. These results are compared with existing data on $\phi$ meson production in p+p collisions. The comparison shows consistency but superior accuracy of the present measurements. The emission of $\phi$ mesons in p+p reactions is confronted with that occurring in Pb+Pb collisions, and the experimental results are compared with model predictions. It appears that none of the considered models can properly describe all the experimental observables.

==> includes/na61Abbreviations.tex <==
%%%%%%% units
\newcommand{\kg}{\ensuremath{\mbox{kg}}\xspace}
\newcommand{\eV}{\ensuremath{\mbox{e\kern-0.1em V}}\xspace}
\newcommand{\GeV}{\ensuremath{\mbox{Ge\kern-0.1em V}}\xspace}
\newcommand{\MeV}{\ensuremath{\mbox{Me\kern-0.1em V}}\xspace}
\newcommand{\GeVc}{\ensuremath{\mbox{Ge\kern-0.1em V}\!/\!c}\xspace}
\newcommand{\GeVcc}{\ensuremath{\mbox{Ge\kern-0.1em V}\!/\!c^2}\xspace}
\newcommand{\AGeV}{\ensuremath{A\,\mbox{Ge\kern-0.1em V}}\xspace}
\newcommand{\AGeVc}{\ensuremath{A\,\mbox{Ge\kern-0.1em V}\!/\!c}\xspace}
\newcommand{\MeVc}{\ensuremath{\mbox{Me\kern-0.1em V}/c}\xspace}
\newcommand{\T}{\ensuremath{\mbox{T}}\xspace}
\newcommand{\cmsq}{\ensuremath{\mbox{cm}^2}\xspace}
\newcommand{\msq}{\ensuremath{\mbox{m}^2}\xspace}
\newcommand{\cm}{\ensuremath{\mbox{cm}}\xspace}
\newcommand{\mm}{\ensuremath{\mbox{mm}}\xspace}
\newcommand{\micron}{\ensuremath{\mu\mbox{m}}\xspace}
\newcommand{\mrad}{\ensuremath{\mbox{mrad}}\xspace}
\newcommand{\ns}{\ensuremath{\mbox{ns}}\xspace}
\newcommand{\m}{\ensuremath{\mbox{m}}\xspace}
\newcommand{\s}{\ensuremath{\mbox{s}}\xspace}
\newcommand{\ms}{\ensuremath{\mbox{ms}}\xspace}
\newcommand{\ps}{\ensuremath{\mbox{ps}}\xspace}
\newcommand{\dd}{\ensuremath{{\rm d}}\xspace}
\newcommand{\dedx}{\ensuremath{\dd E\!/\!\dd x}\xspace}
\newcommand{\tof}{\ensuremath{\textup{\emph{tof}}}\xspace}
\newcommand{\pt}{\ensuremath{p_{\rm T}}\xspace}
\newcommand{\PT}{\ensuremath{P_\textup{T}}\xspace}
\newcommand{\mt}{\ensuremath{m_{\rm T}}\xspace}

%particles
\newcommand{\pbar}{\ensuremath{\overline{\textup{p}}}\xspace}
\newcommand{\pim}{\ensuremath{\pi^-}\xspace}
\newcommand{\pip}{\ensuremath{\pi^+}\xspace}
\newcommand{\km}{\ensuremath{\textup{K}^-}\xspace}
\newcommand{\kp}{\ensuremath{\textup{K}^+}\xspace}
\newcommand{\hm}{\ensuremath{\textup{h}^-}\xspace}

% inverse hyperbolic functions
%\DeclareMathOperator{\acosh}{acosh}
%\DeclareMathOperator{\asinh}{asinh}
%\DeclareMathOperator{\atanh}{atanh}

%%%%%%%%%%%%% some software programs and generators
%----- NA61 software
\def\Offline{\mbox{$\overline{\text%
{Off}}$\hspace{.05em}\raisebox{.4ex}{\underline{line}}}\xspace}
\def\SHOE{\mbox{SHO\hspace{-1.34ex}\raisebox{0.2ex}{\color{green}\textasteriskcentered}\hspace{0.25ex}E}\xspace}
\def\DSHACK{\mbox{DS\hspace{0.15ex}$\hbar$ACK}\xspace}
\DeclareRobustCommand{\SHINE}{\mbox{\textsc{S\hspace{.05em}\raisebox{.4ex}{\underline{hine}}}}\xspace} %DeclareRobustCommand allows this to work in caption
%\def\SHINE{\textsc{Shine}\xspace}
%----- event generators
\def\Glissando{\textsc{Glissando}\xspace}
\newcommand{\FlukaLong}{{\scshape Fluka2008}\xspace}
\newcommand{\FlukaEleven}{{\scshape Fluka2011}\xspace}
\newcommand{\Fluka}{{\scshape Fluka}\xspace}
\newcommand{\UrqmdLong}{{\scshape U}r{\scshape qmd1.3.1}\xspace}
\newcommand{\Urqmd}{{\scshape U}r{\scshape qmd}\xspace}
\newcommand{\GheishaLong}{{\scshape Gheisha2002}\xspace}
\newcommand{\GheishaOld}{{\scshape Gheisha600}\xspace}
\newcommand{\Gheisha}{{\scshape Gheisha}\xspace}
\newcommand{\Corsika}{{\scshape Corsika}\xspace}
\newcommand{\Venus}{{\scshape Venus}\xspace}
\newcommand{\VenusLong}{{\scshape Venus4.12}\xspace}
\newcommand{\GiBUU}{{\scshape GiBUU}\xspace}
\newcommand{\GiBUULong}{{\scshape GiBUU1.6}\xspace}
\newcommand{\FlukaNewLong}{{\scshape Fluka2011.2\_17}\xspace}
\newcommand{\Root}{{\scshape Root}\xspace}
\newcommand{\Geant}{{\scshape Geant}\xspace}
\newcommand{\GeantThree}{{\scshape Geant3}\xspace}
\newcommand{\GeantFour}{{\scshape Geant4}\xspace}
\newcommand{\QGSJet}{{\scshape QGSJet}\xspace}
\newcommand{\DPMJet}{{\scshape DPMJet}\xspace}
\newcommand{\Epos}{{\scshape Epos}\xspace}
\newcommand{\EposLong}{{\scshape Epos1.99}\xspace}
\newcommand{\QGSJetLong}{{\scshape QGSJetII-04}\xspace}
\newcommand{\DPMJetLong}{{\scshape DPMJet3.06}\xspace}
\newcommand{\SibyllLong}{{\scshape Sibyll2.1}\xspace}
\newcommand{\EposLHCLong}{{\scshape EposLHC}\xspace}
\newcommand{\Hsd}{{\scshape Hsd}\xspace}
\newcommand{\Ampt}{{\scshape Ampt}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%% misc
\def\red#1{{\color{red}#1}}
\def\avg#1{\langle{#1}\rangle}
\def\sci#1#2{#1\!\times\!10^{#2}}
\newcommand{\Fi}[1]{Fig.~\ref{#1}}
\newcommand{\CernVM}{\textsc{Cern\-\kern-0.05emVM}\xspace}


==> includes/na61EPJCAuthorsInstitutions.tex <==
\institute{
{National Nuclear Research Center, Baku, Azerbaijan}\label{inst0}
\and{Faculty of Physics, University of Sofia, Sofia, Bulgaria}\label{inst1}
\and{Ru{\dj}er Bo\v{s}kovi\'c Institute, Zagreb, Croatia}\label{inst2}
\and{LPNHE, University of Paris VI and VII, Paris, France}\label{inst3}
\and{Karlsruhe Institute of Technology, Karlsruhe, Germany}\label{inst4}
\and{University of Frankfurt, Frankfurt, Germany}\label{inst5}
\and{Wigner Research Centre for Physics of the Hungarian Academy of Sciences, Budapest, Hungary}\label{inst6}
\and{University of Bergen, Bergen, Norway}\label{inst7}
\and{Jan Kochanowski University in Kielce, Poland}\label{inst8}
\and{Institute of Nuclear Physics, Polish Academy of Sciences, Cracow, Poland}\label{inst9}
\and{National Centre for Nuclear Research, Warsaw, Poland}\label{inst10}
\and{Jagiellonian University, Cracow, Poland}\label{inst11}
\and{AGH - University of Science and Technology, Cracow, Poland}\label{inst12}
\and{University of Silesia, Katowice, Poland}\label{inst13}
\and{University of Warsaw, Warsaw, Poland}\label{inst14}
\and{University of Wroc{\l}aw,  Wroc{\l}aw, Poland}\label{inst15}
\and{Warsaw University of Technology, Warsaw, Poland}\label{inst16}
\and{Institute for Nuclear Research, Moscow, Russia}\label{inst17}
\and{Joint Institute for Nuclear Research, Dubna, Russia}\label{inst18}
\and{National Research Nuclear University (Moscow Engineering Physics Institute), Moscow, Russia}\label{inst19}
\and{St. Petersburg State University, St. Petersburg, Russia}\label{inst20}
\and{University of Belgrade, Belgrade, Serbia}\label{inst21}
\and{University of Geneva, Geneva, Switzerland}\label{inst22}
\and{Fermilab, Batavia, USA}\label{inst23}
\and{University of Colorado, Boulder, USA}\label{inst24}
\and{University of Pittsburgh, Pittsburgh, USA}\label{inst25}
}
\author{
  {\bf The NA61/SHINE Collaboration:\\[1ex]}
{A.~Aduszkiewicz}\thanksref{inst14}
\and{E.V.~Andronov}\thanksref{inst20}
\and{T.~Anti\'ci\'c}\thanksref{inst2}
\and{V.~Babkin}\thanksref{inst18}
\and{M.~Baszczyk}\thanksref{inst12}
\and{S.~Bhosale}\thanksref{inst9}
\and{A.~Blondel}\thanksref{inst22}
\and{M.~Bogomilov}\thanksref{inst1}
\and{A.~Brandin}\thanksref{inst19}
\and{A.~Bravar}\thanksref{inst22}
\and{W.~Bryli\'nski}\thanksref{inst16}
\and{J.~Brzychczyk}\thanksref{inst11}
\and{M.~Buryakov}\thanksref{inst18}
\and{O.~Busygina}\thanksref{inst17}
\and{A.~Bzdak}\thanksref{inst12}
\and{H.~Cherif}\thanksref{inst5}
\and{M.~\'Cirkovi\'c}\thanksref{inst21}
\and{~M.~Csanad~}\thanksref{inst6}
\and{J.~Cybowska}\thanksref{inst16}
\and{T.~Czopowicz}\thanksref{inst16}
\and{A.~Damyanova}\thanksref{inst22}
\and{N.~Davis}\thanksref{inst9}
\and{M.~Deliyergiyev}\thanksref{inst8}
\and{M.~Deveaux}\thanksref{inst5}
\and{A.~Dmitriev~}\thanksref{inst18}
\and{W.~Dominik}\thanksref{inst14}
\and{P.~Dorosz}\thanksref{inst12}
\and{J.~Dumarchez}\thanksref{inst3}
\and{R.~Engel}\thanksref{inst4}
\and{G.A.~Feofilov}\thanksref{inst20}
\and{L.~Fields}\thanksref{inst23}
\and{Z.~Fodor}\thanksref{inst6, inst15}
\and{A.~Garibov}\thanksref{inst0}
\and{M.~Ga\'zdzicki}\thanksref{inst5, inst8}
\and{O.~Golosov}\thanksref{inst19}
\and{V.~Golovatyuk~}\thanksref{inst18}
\and{M.~Golubeva}\thanksref{inst17}
\and{K.~Grebieszkow}\thanksref{inst16}
\and{F.~Guber}\thanksref{inst17}
\and{A.~Haesler}\thanksref{inst22}
\and{S.N.~Igolkin}\thanksref{inst20}
\and{S.~Ilieva}\thanksref{inst1}
\and{A.~Ivashkin}\thanksref{inst17}
\and{S.R.~Johnson}\thanksref{inst24}
\and{K.~Kadija}\thanksref{inst2}
\and{E.~Kaptur}\thanksref{inst13}
\and{N.~Kargin}\thanksref{inst19}
\and{E.~Kashirin}\thanksref{inst19}
\and{M.~Kie{\l}bowicz}\thanksref{inst9}
\and{V.A.~Kireyeu}\thanksref{inst18}
\and{V.~Klochkov}\thanksref{inst5}
\and{V.I.~Kolesnikov}\thanksref{inst18}
\and{D.~Kolev}\thanksref{inst1}
\and{A.~Korzenev}\thanksref{inst22}
\and{V.N.~Kovalenko}\thanksref{inst20}
\and{K.~Kowalik}\thanksref{inst10}
\and{S.~Kowalski}\thanksref{inst13}
\and{M.~Koziel}\thanksref{inst5}
\and{A.~Krasnoperov}\thanksref{inst18}
\and{W.~Kucewicz}\thanksref{inst12}
\and{M.~Kuich}\thanksref{inst14}
\and{A.~Kurepin}\thanksref{inst17}
\and{D.~Larsen}\thanksref{inst11}
\and{A.~L\'aszl\'o}\thanksref{inst6}
\and{T.V.~Lazareva}\thanksref{inst20}
\and{M.~Lewicki}\thanksref{inst15}
\and{K.~{\L}ojek}\thanksref{inst11}
\and{B.~{\L}ysakowski}\thanksref{inst13}
\and{V.V.~Lyubushkin}\thanksref{inst18}
\and{M.~Ma\'ckowiak-Paw{\l}owska}\thanksref{inst16}
\and{Z.~Majka}\thanksref{inst11}
\and{B.~Maksiak}\thanksref{inst10}
\and{A.I.~Malakhov}\thanksref{inst18}
\and{D.~Mani\'c}\thanksref{inst21}
\and{A.~Marchionni}\thanksref{inst23}
\and{A.~Marcinek}\thanksref{inst9,e1}
\and{A.D.~Marino}\thanksref{inst24}
\and{K.~Marton}\thanksref{inst6}
\and{H.-J.~Mathes}\thanksref{inst4}
\and{T.~Matulewicz}\thanksref{inst14}
\and{V.~Matveev}\thanksref{inst18}
\and{G.L.~Melkumov}\thanksref{inst18}
\and{A.O.~Merzlaya}\thanksref{inst11}
\and{B.~Messerly}\thanksref{inst25}
\and{{\L}.~Mik}\thanksref{inst12}
\and{S.~Morozov}\thanksref{inst17, inst19}
\and{S.~Mr\'owczy\'nski}\thanksref{inst8}
\and{Y.~Nagai}\thanksref{inst24}
\and{M.~Naskr\k{e}t}\thanksref{inst15}
\and{V.~Ozvenchuk}\thanksref{inst9}
\and{V.~Paolone}\thanksref{inst25}
\and{M.~Pavin}\thanksref{inst3, inst2}
\and{O.~Petukhov}\thanksref{inst17}
\and{R.~P{\l}aneta}\thanksref{inst11}
\and{P.~Podlaski}\thanksref{inst14}
\and{B.A.~Popov}\thanksref{inst18, inst3}
\and{B.~Porfy}\thanksref{inst6}
\and{M.~Posiada{\l}a-Zezula}\thanksref{inst14}
\and{D.S.~Prokhorova}\thanksref{inst20}
\and{D.~Pszczel}\thanksref{inst10}
\and{S.~Pu{\l}awski}\thanksref{inst13}
\and{J.~Puzovi\'c}\thanksref{inst21}
\and{M.~Ravonel}\thanksref{inst22}
\and{R.~Renfordt}\thanksref{inst5}
\and{E.~Richter-W\k{a}s}\thanksref{inst11}
\and{D.~R\"ohrich}\thanksref{inst7}
\and{E.~Rondio}\thanksref{inst10}
\and{M.~Roth}\thanksref{inst4}
\and{B.T.~Rumberger}\thanksref{inst24}
\and{M.~Rumyantsev}\thanksref{inst18}
\and{A.~Rustamov}\thanksref{inst0, inst5}
\and{M.~Rybczynski}\thanksref{inst8}
\and{A.~Rybicki}\thanksref{inst9}
\and{A.~Sadovsky}\thanksref{inst17}
\and{K.~Schmidt}\thanksref{inst13}
\and{I.~Selyuzhenkov}\thanksref{inst19}
\and{A.Yu.~Seryakov}\thanksref{inst20}
\and{P.~Seyboth}\thanksref{inst8}
\and{M.~S{\l}odkowski}\thanksref{inst16}
\and{P.~Staszel}\thanksref{inst11}
\and{G.~Stefanek}\thanksref{inst8}
\and{J.~Stepaniak}\thanksref{inst10}
\and{M.~Strikhanov}\thanksref{inst19}
\and{H.~Str\"obele}\thanksref{inst5}
\and{T.~\v{S}u\v{s}a}\thanksref{inst2}
\and{A.~Taranenko}\thanksref{inst19}
\and{A.~Tefelska}\thanksref{inst16}
\and{D.~Tefelski}\thanksref{inst16}
\and{V.~Tereshchenko}\thanksref{inst18}
\and{A.~Toia}\thanksref{inst5}
\and{R.~Tsenov}\thanksref{inst1}
\and{L.~Turko}\thanksref{inst15}
\and{R.~Ulrich}\thanksref{inst4}
\and{M.~Unger}\thanksref{inst4}
\and{F.F.~Valiev}\thanksref{inst20}
\and{D.~Veberi\v{c}}\thanksref{inst4}
\and{V.V.~Vechernin}\thanksref{inst20}
\and{A.~Wickremasinghe}\thanksref{inst25}
\and{Z.~W{\l}odarczyk}\thanksref{inst8}
\and{A.~Wojtaszek-Szwarc}\thanksref{inst8}
\and{O.~Wyszy\'nski}\thanksref{inst11}
\and{L.~Zambelli}\thanksref{inst3}
\and{E.D.~Zimmerman}\thanksref{inst24}
\and{R.~Zwaska}\thanksref{inst23}
}

\authorrunning{NA61/SHINE Collaboration}


==> tables/pp158_Tmt.tex <==
142 \pm 10 \pm 9


==> tables/pp158_pt_sigma_y.tex <==
% p_{T} [GeV/c]      & #sigma_{y}                
% min max            & value    stat    syst     
  0.0--0.2           & $1.19 \pm 0.16 \pm 0.18$   \\
  0.2--0.4           & $0.967 \pm 0.059 \pm 0.046$ \\
  0.4--0.6           & $0.930 \pm 0.049 \pm 0.046$ \\
  0.6--0.8           & $0.853 \pm 0.052 \pm 0.039$ \\
  0.8--1.2           & $0.945 \pm 0.074 \pm 0.062$ \\
  1.2--1.6           & $0.82 \pm 0.12 \pm 0.06$   \\


==> tables/pp158_y.tex <==
% y            & dn/dy                     
% min max      & value    stat    syst     
  0.0--0.3     & $0.00558 \pm 0.00037 \pm 0.00031$ \\
  0.3--0.6     & $0.00453 \pm 0.00021 \pm 0.00016$ \\
  0.6--0.9     & $0.00394 \pm 0.00020 \pm 0.00016$ \\
  0.9--1.5     & $0.00222 \pm 0.00011 \pm 0.00011$ \\
  1.5--2.1     & $0.000955 \pm 0.000089 \pm 0.000071$ \\


==> tables/pp158_y_T.tex <==
% y            & T [MeV]                   
% min max      & value    stat    syst     
  0.0--0.3     & $147 \pm 11 \pm 8$         \\
  0.3--0.6     & $152.5 \pm 8.2 \pm 5.8$    \\
  0.6--0.9     & $159.3 \pm 7.6 \pm 4.9$    \\
  0.9--1.5     & $144.6 \pm 7.1 \pm 5.9$    \\
  1.5--2.1     & $129 \pm 15 \pm 10$        \\


==> tables/pp158_y_mt.tex <==
% y            & m_{T} - m_{0}  [GeV/c^{2}]      & d^{2}n/(m_{T}dm_{T}dy)  [(GeV/c^{2})^{-2}]     
% min max      & min  max                        & value    stat    syst                          
  0.0--0.3     & 0.00--0.05                      & $0.0305 \pm 0.0036 \pm 0.0038$                  \\
  0.0--0.3     & 0.05--0.10                      & $0.0188 \pm 0.0028 \pm 0.0024$                  \\
  0.0--0.3     & 0.10--0.20                      & $0.0128 \pm 0.0017 \pm 0.0018$                  \\
  0.0--0.3     & 0.20--0.30                      & $0.0066 \pm 0.0011 \pm 0.0013$                  \\
  0.0--0.3     & 0.30--0.50                      & $0.00223 \pm 0.00048 \pm 0.00031$               \\
  0.0--0.3     & 0.50--0.70                      & $0.00049 \pm 0.00023 \pm 0.00021$               \\


==> tables/pp158_y_pt.tex <==
% y            & p_{T} [GeV/c]      & d^{2}n/(dp_{T}dy)  [(GeV/c)^{-1}]     
% min max      & min  max           & value    stat    syst                 
  0.0--0.3     & 0.0--0.2           & $0.00341 \pm 0.00058 \pm 0.00051$      \\
  0.0--0.3     & 0.2--0.4           & $0.00744 \pm 0.00088 \pm 0.00085$      \\
  0.0--0.3     & 0.4--0.6           & $0.00619 \pm 0.00091 \pm 0.00074$      \\
  0.0--0.3     & 0.6--0.8           & $0.00547 \pm 0.00084 \pm 0.00074$      \\
  0.0--0.3     & 0.8--1.2           & $0.00219 \pm 0.00037 \pm 0.00028$      \\
  0.0--0.3     & 1.2--1.6           & $0.00046 \pm 0.00020 \pm 0.00009$      \\
  0.3--0.6     & 0.0--0.2           & $0.00217 \pm 0.00032 \pm 0.00041$      \\
  0.3--0.6     & 0.2--0.4           & $0.00534 \pm 0.00048 \pm 0.00032$      \\
  0.3--0.6     & 0.4--0.6           & $0.00645 \pm 0.00055 \pm 0.00032$      \\
  0.3--0.6     & 0.6--0.8           & $0.00453 \pm 0.00047 \pm 0.00029$      \\
  0.3--0.6     & 0.8--1.2           & $0.00145 \pm 0.00023 \pm 0.00019$      \\
  0.3--0.6     & 1.2--1.6           & $0.00057 \pm 0.00014 \pm 0.00006$      \\
  0.6--0.9     & 0.0--0.2           & $0.00114 \pm 0.00028 \pm 0.00011$      \\
  0.6--0.9     & 0.2--0.4           & $0.00534 \pm 0.00050 \pm 0.00041$      \\
  0.6--0.9     & 0.4--0.6           & $0.00530 \pm 0.00050 \pm 0.00043$      \\
  0.6--0.9     & 0.6--0.8           & $0.00378 \pm 0.00043 \pm 0.00035$      \\
  0.6--0.9     & 0.8--1.2           & $0.00167 \pm 0.00020 \pm 0.00018$      \\
  0.6--0.9     & 1.2--1.6           & $0.000316 \pm 0.000089 \pm 0.000040$   \\
  0.9--1.5     & 0.0--0.2           & $0.00130 \pm 0.00018 \pm 0.00015$      \\
  0.9--1.5     & 0.2--0.4           & $0.00274 \pm 0.00027 \pm 0.00035$      \\
  0.9--1.5     & 0.4--0.6           & $0.00304 \pm 0.00029 \pm 0.00029$      \\
  0.9--1.5     & 0.6--0.8           & $0.00204 \pm 0.00023 \pm 0.00025$      \\
  0.9--1.5     & 0.8--1.2           & $0.00081 \pm 0.00010 \pm 0.00008$      \\
  0.9--1.5     & 1.2--1.6           & $0.000168 \pm 0.000047 \pm 0.000032$   \\
  1.5--2.1     & 0.0--0.2           & $0.00077 \pm 0.00016 \pm 0.00011$      \\
  1.5--2.1     & 0.2--0.4           & $0.00139 \pm 0.00024 \pm 0.00015$      \\
  1.5--2.1     & 0.4--0.6           & $0.00114 \pm 0.00021 \pm 0.00023$      \\
  1.5--2.1     & 0.6--0.8           & $0.00062 \pm 0.00018 \pm 0.00012$      \\
  1.5--2.1     & 0.8--1.2           & $0.000355 \pm 0.000088 \pm 0.000079$   \\
  1.5--2.1     & 1.2--1.6           & $0.000066 \pm 0.000034 \pm 0.000016$   \\


==> tables/pp40_Tpt.tex <==
128.0 \pm 9.3 \pm 8.0


==> tables/pp40_y.tex <==
% y            & dn/dy                     
% min max      & value    stat    syst     
  0.0--0.3     & $0.00278 \pm 0.00040 \pm 0.00052$ \\
  0.3--0.6     & $0.00254 \pm 0.00028 \pm 0.00028$ \\
  0.6--0.9     & $0.00197 \pm 0.00021 \pm 0.00021$ \\
  0.9--1.2     & $0.00136 \pm 0.00015 \pm 0.00024$ \\
  1.2--1.5     & $0.00059 \pm 0.00012 \pm 0.00013$ \\


==> tables/pp40_y_pt.tex <==
% y            & p_{T} [GeV/c]      & d^{2}n/(dp_{T}dy)  [(GeV/c)^{-1}]     
% min max      & min  max           & value    stat    syst                 
  0.0--1.5     & 0.0--0.2           & $0.00151 \pm 0.00017 \pm 0.00020$      \\
  0.0--1.5     & 0.2--0.4           & $0.00258 \pm 0.00026 \pm 0.00033$      \\
  0.0--1.5     & 0.4--0.6           & $0.00205 \pm 0.00029 \pm 0.00030$      \\
  0.0--1.5     & 0.6--0.8           & $0.00155 \pm 0.00026 \pm 0.00025$      \\
  0.0--1.5     & 0.8--1.4           & $0.000508 \pm 0.000080 \pm 0.000057$   \\


==> tables/pp80_Tmt.tex <==
146 \pm 19 \pm 18


==> tables/pp80_pt_sigma_y.tex <==
% p_{T} [GeV/c]      & #sigma_{y}                
% min max            & value    stat    syst     
  0.0--0.2           & $0.86 \pm 0.10 \pm 0.08$   \\
  0.2--0.4           & $0.929 \pm 0.091 \pm 0.078$ \\
  0.4--0.6           & $0.96 \pm 0.11 \pm 0.09$   \\
  0.6--0.8           & $0.87 \pm 0.13 \pm 0.11$   \\
  0.8--1.2           & $0.689 \pm 0.061 \pm 0.043$ \\


==> tables/pp80_y.tex <==
% y            & dn/dy                     
% min max      & value    stat    syst     
  0.0--0.3     & $0.00323 \pm 0.00029 \pm 0.00029$ \\
  0.3--0.6     & $0.00336 \pm 0.00022 \pm 0.00020$ \\
  0.6--0.9     & $0.00284 \pm 0.00018 \pm 0.00016$ \\
  0.9--1.5     & $0.001351 \pm 0.000092 \pm 0.000073$ \\


==> tables/pp80_y_T.tex <==
% y            & T [MeV]                   
% min max      & value    stat    syst     
  0.0--0.3     & $150 \pm 18 \pm 18$        \\
  0.3--0.6     & $139 \pm 13 \pm 10$        \\
  0.6--0.9     & $138 \pm 13 \pm 9$         \\
  0.9--1.5     & $119.0 \pm 9.5 \pm 7.2$    \\


==> tables/pp80_y_mt.tex <==
% y            & m_{T} - m_{0}  [GeV/c^{2}]      & d^{2}n/(m_{T}dm_{T}dy)  [(GeV/c^{2})^{-2}]     
% min max      & min  max                        & value    stat    syst                          
  0.0--0.3     & 0.00--0.05                      & $0.0170 \pm 0.0023 \pm 0.0036$                  \\
  0.0--0.3     & 0.05--0.10                      & $0.0100 \pm 0.0020 \pm 0.0018$                  \\
  0.0--0.3     & 0.10--0.20                      & $0.0050 \pm 0.0012 \pm 0.0010$                  \\
  0.0--0.3     & 0.20--0.30                      & $0.00438 \pm 0.00099 \pm 0.00078$               \\
  0.0--0.3     & 0.30--0.50                      & $0.00131 \pm 0.00036 \pm 0.00023$               \\


==> tables/pp80_y_pt.tex <==
% y            & p_{T} [GeV/c]      & d^{2}n/(dp_{T}dy)  [(GeV/c)^{-1}]     
% min max      & min  max           & value    stat    syst                 
  0.0--0.3     & 0.0--0.2           & $0.00223 \pm 0.00040 \pm 0.00055$      \\
  0.0--0.3     & 0.2--0.4           & $0.00424 \pm 0.00064 \pm 0.00096$      \\
  0.0--0.3     & 0.4--0.6           & $0.00303 \pm 0.00070 \pm 0.00063$      \\
  0.0--0.3     & 0.6--0.8           & $0.00309 \pm 0.00069 \pm 0.00049$      \\
  0.0--0.3     & 0.8--1.2           & $0.00150 \pm 0.00032 \pm 0.00022$      \\
  0.3--0.6     & 0.0--0.2           & $0.00167 \pm 0.00031 \pm 0.00021$      \\
  0.3--0.6     & 0.2--0.4           & $0.00481 \pm 0.00052 \pm 0.00048$      \\
  0.3--0.6     & 0.4--0.6           & $0.00492 \pm 0.00058 \pm 0.00067$      \\
  0.3--0.6     & 0.6--0.8           & $0.00179 \pm 0.00047 \pm 0.00022$      \\
  0.3--0.6     & 0.8--1.2           & $0.00157 \pm 0.00028 \pm 0.00023$      \\
  0.6--0.9     & 0.0--0.2           & $0.00219 \pm 0.00031 \pm 0.00020$      \\
  0.6--0.9     & 0.2--0.4           & $0.00333 \pm 0.00044 \pm 0.00061$      \\
  0.6--0.9     & 0.4--0.6           & $0.00381 \pm 0.00042 \pm 0.00034$      \\
  0.6--0.9     & 0.6--0.8           & $0.00186 \pm 0.00035 \pm 0.00015$      \\
  0.6--0.9     & 0.8--1.2           & $0.00131 \pm 0.00021 \pm 0.00011$      \\
  0.9--1.5     & 0.0--0.2           & $0.00080 \pm 0.00016 \pm 0.00011$      \\
  0.9--1.5     & 0.2--0.4           & $0.00211 \pm 0.00024 \pm 0.00020$      \\
  0.9--1.5     & 0.4--0.6           & $0.00199 \pm 0.00025 \pm 0.00018$      \\
  0.9--1.5     & 0.6--0.8           & $0.00100 \pm 0.00019 \pm 0.00016$      \\
  0.9--1.5     & 0.8--1.2           & $0.000380 \pm 0.000087 \pm 0.000064$   \\

